The Shapley Value of Inconsistency Measures for Functional Dependencies

Quantifying the inconsistency of a database is motivated by various goals including reliability estimation for new datasets and progress indication in data cleaning. Another goal is to attribute to individual tuples a level of responsibility to the overall inconsistency, and thereby prioritize tuples in the explanation or inspection of dirt. Therefore, inconsistency quantification and attribution have been a subject of much research in Knowledge Representation and, more recently, in Databases. As in many other fields, a conventional responsibility sharing mechanism is the Shapley value from cooperative game theory. In this paper, we carry out a systematic investigation of the complexity of the Shapley value in common inconsistency measures for functional-dependency (FD) violations. For several measures we establish a full classification of the FD sets into tractable and intractable classes with respect to Shapley-value computation. We also study the complexity of approximation in intractable cases.

==> minimal_inconsistent.tex <==
\section{Number of Minimal Inconsistent Subsets}

In this section, we consider the measure $\Imi$, that counts the number of \e{minimal inconsistent subsets} (i.e., pairs of tuples that jointly violate at least one FD). 
An easy observation is that a fact $f$ increases the value of the measure $\Imi$ by $i$ in a permutation $\sigma$ if and only if $\sigma_f$ contains exactly $i$ facts that are in conflict with $f$. Hence, the Shapley value for this measure can be computed in the following way.
$$\shapley(D,\depset,f,\Imi)=\frac{1}{|D|!}\sum_{i=1}^{n}\sum_{k=i}^{|D|-1}{n \choose i}{|D|-n \choose k-i} k!\cdot (|D|-k-1)!\cdot i$$
where $n$ is the number of facts in $D$ that are in conflict with $f$.

Therefore, we immediately obtain the following result.

\begin{theorem}
  Let $\depset$ be a set of FDs. Computing $\shapley(D,\depset,f,\Imi)$ can be done in polynomial time, given $D$ and $f$.
\end{theorem}

==> problematic.tex <==
\section{Number of Problematic Facts}\label{sec:problematic}

We now consider the measure $\Ip$ that counts the number of ``problematic'' tuples; that is, tuples that participate in a violation of $\depset$.
A fact $f$ increases the measure by $m$ in a permutation $\sigma$ if and only if $\sigma_f$ contains precisely $m-1$ facts that are in conflict with $f$, but not in conflict with any other fact of $\sigma_f$ (hence, all these facts and $f$ itself are added to the group of problematic facts).

 We prove the following.
 
 \begin{theorem}\label{thm:ponefd}
Let $\depset$ be a set of FDs. Computing $\shapley(D,f,\Ip,\depset)$ can be done in polynomial time, given $D$ and $f$.
\end{theorem}
\begin{proof}
We now show how the values $\Exp_{D'\sim U_m(D)}\big(\Ip(D',\depset)\big)$ and $\Exp_{D'\sim U_m(D)}\big(\Ip(D'\cup\set{f},\depset)\big)$ can be computed in polynomial time. We start with the first value.

We denote by $X_m$ a random variable holding the number of problematic facts in a subset of size $m$ of $D$, and by $X_m^g$ a random variable that holds $1$ if the fact $g$ is selected and participates in a violation of the FDs in a subset of size $m$ of $D$, and $0$ otherwise.
We have the following.

\begin{align*}%\label{eq:shapley-bcq}
  \Exp_{D'\sim U_m(D)}\big(\Ip(D',\depset)\big)&=\Exp(X_m)=\Exp(\sum_{g\in {D\setminus\set{f}}}X_m^g)=\sum_{g\in {D\setminus\set{f}}}\Exp(X_m^g)
\end{align*}
Hence, the computation of $\Exp_{D'\sim U_m(D)}\big(\Ip(D',\depset)\big)$ reduces to the computation of $\Exp(X_m^g)$. This value can be computed as follows.

\begin{align*}%\label{eq:shapley-bcq}
  \Exp(X_m^g)&=\Pr{g\mbox{ is selected in a subset of size }m}\\
  &\cdot\Pr{\mbox{a conflicting fact is selected in a subset of size }m\mid g\mbox{ is selected in the subset}}\\
  &=\frac{{{|D|-2}\choose {m-1}}}{{{|D|-1}\choose m}}\cdot \frac{\sum_{k=1}^{N_g}{{N_g}\choose k}\cdot {{|D|-1-N_g}\choose{m-k-1}}}{{{|D|-2}\choose {m-1}}}=\frac{\sum_{k=1}^{N_g}{{N_g}\choose k}\cdot {{|D|-1-N_g}\choose{m-k-1}}}{{{|D|-1}\choose m}}
\end{align*}
where $N_g$ is the number of facts in $D\setminus\set{f}$ that are in conflict with $g$.

Similarly, we can compute:

\begin{align*}%\label{eq:shapley-bcq}
  \Exp_{D'\sim U_m(D)}\big(\Ip(D'\cup\set{f},\depset)\big)&=\Exp(X_{m,f})=\Exp(\sum_{g\in {D\setminus\set{f}}}X_{m,f}^g)=\sum_{g\in {D\setminus\set{f}}}\Exp(X_{m,f}^g)
\end{align*}
where $X_{m,f}$ is a random variable holding the number of problematic facts in a subset of size $m$ of $D\setminus\set{f}$ after adding the fact $f$, and $X_{m,f}^g$ is a random variable that holds $1$ if $g$ is selected in such a subset and violates the FDs with another fact from the subset and $0$ otherwise.

For a fact $g$ that is not in conflict with $f$ we have that:
\begin{align*}%\label{eq:shapley-bcq}
  \Exp(X_{m,f}^g)&=\Exp(X_m^g)
\end{align*}
while for a fact $g$ that is in conflict with $f$ we have that:
\begin{align*}%\label{eq:shapley-bcq}
  \Exp(X_{m,f}^g)&=\Pr{g\mbox{ is selected in a subset of size }m}=\frac{{{|D|-2}\choose {m-1}}}{{{|D|-1}\choose m}}
\end{align*}
and that concludes our proof.
\end{proof}


